DP-RuL: Differentially-Private Rule Learning for Clinical Decision Support Systems

Serious privacy concerns arise with the use of patient data in rule-based clinical decision support systems (CDSS). The goal of a privacy-preserving CDSS is to learn a population ruleset from individual clients' local rulesets, while protecting the potentially sensitive information contained in the rulesets. We present the first work focused on this problem and develop a framework for learning population rulesets with local differential privacy (LDP), suitable for use within a distributed CDSS and other distributed settings. Our rule discovery protocol uses a Monte-Carlo Tree Search (MCTS) method integrated with LDP to search a rule grammar in a structured way and find rule structures clients are likely to have. Randomized response queries are sent to clients to determine promising paths to search within the rule grammar. In addition, we introduce an adaptive budget allocation method which dynamically determines how much privacy loss budget to use at each query, resulting in better privacy-utility trade-offs. We evaluate our approach using three clinical datasets and find that we are able to learn population rulesets with high coverage (breadth of rules) and clinical utility even at low privacy loss budgets.

==> Adaptive_Budget_Prev_Versions.tex <==

% \textbf{Adaptive.} The core idea behind the adaptive budget is this: At each query, adaptively determine $\beta$: add the maximum amount of noise (or alternatively, minimize the budget used).

% We want to find the minimum budget value $\beta$ that ensures that:
% $$P[|c - \hat{c}| \leq d ]\geq 95\%$$ where $\hat{c}$ is the estimated count, $c$ is the true count and $d$ is a user specified distance. In other words, we wish to ensure with 95\% probability that the difference (distance) between the the true count $c$ and the estimated count $\hat{c}$ is within some distance $d$. This essentially provides a way to find a budget that bounds the error between the observed and ground truth counts. We use $c$ from the previous node. If there is no parent node, we assume $c = 0.5 \times n$.

% We assume a gaussian distribution, and we can estimate the observed mean count as: 
% $$\hat{c} = p \times n$$ 
% and the standard deviation as: 
% $$\sigma = \frac{nq(1-q)}{(p-q)^2}$$ 

% To compute the probability that an estimated count is some distance from the ground truth count, we first compute z-scores for the upper and lower distances:
% $$z_{upper} = \frac{\hat{c} - c + d}{\sigma}$$
% $$z_{lower} = \frac{\hat{c} - c - d}{\sigma}$$

% Then, we can use the cumulative distribution function (CDF) to find the probability that the estimated count falls within +/- $d$ of the true count:
% $$P[c - d \leq \hat{c} \leq c + d] = [CDF(z_{upper}) - CDF(z_{lower})]$$

% Finally we use a nonlinear programming solver to find an approximate minimum $\beta$ that solves this equation:
% $$[CDF(z_{upper}) - CDF(z_{lower})] \geq 0.95$$

% We set $d = 2 * \sigma$ and use the python package Gekko to solve the problem.

% \newpage
% \textbf{Adaptive V2}
% In the basic randomized response protocol, a user $i$ outputs a response $r_i$, which is equal to "yes" or heads with value $$p = \frac{e^\beta}{1 + e^\beta}$$ and "no" or tails with probability q (uniformly at random):
% $$q = 1-p = \frac{1}{1 + e^\beta}$$

% For the adaptive budget, our goal is to maximize the number of queries we complete before running out of budget. Therefore, at each query, we wish to find the minimum budget value $\beta$ that ensures that:
% $$P[|c - \hat{c}| \leq d ]\geq 95\%$$ where $\hat{c}$ is the estimated count, $c$ is the true count and $d$ is a user specified distance. In other words, we wish to ensure with 95\% probability that the difference (distance) between the the true count $c$ and the estimated count $\hat{c}$ is within some distance $d$. 
% % This essentially provides a way to find a budget that bounds the error between the observed and ground truth counts. We use $c$ from the previous node. If there is no parent node, we assume $c = 0.5 \times n$.

% We use $c$ from the previous node. If there is no parent node, we assume $c = 0.5 \times n$.

% We estimate the observed mean count as: 
% $$\hat{c} = p \times n$$ 
% and the standard deviation as: 
% $$\sigma = \frac{nq(1-q)}{(p-q)^2}$$ 

% To solve this problem, we can formulate our equation as:
% $$P[|c - \hat{c}| \leq d ] = P[c - d \leq \hat{c} \leq c + d]$$ 
% (Basically ensure that $\hat{c}$ is bounded by our distances.)

% Therefore, our minimization problem is as follows:
% $$\min_{\beta} \quad P[c - d \leq \hat{c} \leq c + d] \geq 0.95$$
% $$\min_{\beta} \quad P[c - d \leq \left(\frac{e^\beta}{1 + e^\beta} \times n\right) \leq c + d] \geq 0.95$$

% To solve this we do the following: 
% To compute the probability that an estimated count is some distance from the ground truth count, we first compute z-scores for the upper and lower distances:
% $$z_{upper} = \frac{\hat{c} - c + d}{\sigma}$$
% $$z_{lower} = \frac{\hat{c} - c - d}{\sigma}$$

% Then, we can use the cumulative distribution function (CDF) to find the probability that the estimated count falls within +/- $d$ of the true count:
% $$P[c - d \leq \hat{c} \leq c + d] = [CDF(z_{upper}) - CDF(z_{lower})]$$

% Finally we use a nonlinear programming solver to find an approximate minimum $\beta$ that solves this equation:
% $$[CDF(z_{upper}) - CDF(z_{lower})] \geq 0.95$$


% The motivation here is that we wish to perform as many queries as possible.
% For the adaptive budget, our goal is to maximize the number of queries we complete before running out of budget.
% Specifically, we wish to bound the probability that we make an incorrect decision in our search, namely continue searching down a path when we should have stopped (cut off the branch) or cutoff a branch when we actually should have kept searching down it.

% Therefore, at each query, we wish to find the minimum budget value $\beta$ that ensures that:
% If $c \leq \lambda$:
% $$P[c - \lambda \geq \hat{c} - \lambda ] \geq \theta$$
% Where $\theta$ is a hyperparameter specifying the probability bound (e.g., 95\%).
 

% \textbf{Adaptive V3}
% For the adaptive budget, our goal is to maximize the number of queries we complete before running out of budget, while bounding the probability that we make an incorrect choice: specifically, cutoff a branch when we should not have, or continue down a branch when we should have cut it off. Therefore, at each query given an estimated mean count $\hat{c}$, the true mean count $c$ and our cutoff threshold $\lambda$, we want to ensure that:
% $$P[\hat{c} > \lambda \;\lvert\; c \leq \lambda] + P[\hat{c} \leq \lambda \;\lvert\; c > \lambda] \leq \theta$$
% where $\theta$ is a hyperparameter specifying the error probability bound (e.g., 5\%).

% We assume Gaussian distributions for the counts (ref Tianhao's paper here about how this is justified). We use $c$ from the previous node. If there is no parent node, we assume $c = 0.5 \times n$.
% We estimate the observed mean count as: 
% $$\hat{c} = p \times n$$ 

% Given $q$, we can compute the standard deviation as: 
% $$\sigma = \frac{q(1-q)}{n(p-q)^2}$$ 

% To compute the probability that a mean count $v$ is less than or equal to the cutoff threshold $\lambda$: we can use Cumulative Distribution Functions (CDFs), denoted as $\Phi$: 
% $$P(v \leq \lambda)=\Phi(z(v))$$
% where $Z$ is a transformation of the our specific value's Gaussian distributions to the standard normal distribution: 
% $$Z(v) = \frac{\lambda - v}{\sigma_v}$$
% and $\sigma_v$ is the standard deviation of $v$


% Therefore, we can compute the probabilities as:
% $$P(\hat{c} > \lambda) = 1 - \Phi(Z(\hat{c}))$$
% $$P(c \leq \lambda) = \Phi(Z(c))$$
% $$P(\hat{c} \leq \lambda) = \Phi(Z(\hat{c}))$$
% $$P(c > \lambda) = 1 - \Phi(Z(c))$$

% Then we can compute the conditional probabilities as:
% $$P[\hat{c} > \lambda \;\lvert\; c \leq \lambda] = \frac{P(\hat{c} > \lambda)}{P(c \leq \lambda)} 
% = \frac{1 - \Phi(Z(\hat{c}))}{\Phi(Z(c))} $$
% $$P[\hat{c} \leq \lambda \;\lvert\; c > \lambda] = \frac{P(\hat{c} \leq \lambda)}{P(c > \lambda)} 
% = \frac{\Phi(Z(\hat{c}))}{1 - \Phi(Z(c))}$$

% Putting it all together:
% \begin{align*} 
% &P[\hat{c} > \lambda \;\lvert\; c \leq \lambda] + P[\hat{c} \leq \lambda \;\lvert\; c > \lambda]  \\ 
% &= \frac{1 - \Phi(Z(\hat{c}))}{\Phi(Z(c))} + \frac{\Phi(Z(\hat{c}))}{1 - \Phi(Z(c))}
% \end{align*}


% Adaptive V5
\textbf{Before query sent: estimate budget $\beta$ to use}
% Before query: Estimate $\beta$ adaptive budget
Before we send our next query: find the optimal budget per query $\beta$ that allows us to prune branches with high confidence.
Given $\mathcal{A}$, the set of active clients, the unknown true count of yes responses $c$, and the valid rule threshold $\mathcal{V}$, %cutoff threshold $\lambda$,
we can get an estimate count of yes responses $\hat{c}$ based on a selected $\beta$:
$$\hat{c} = y \times p + (\mathcal{A} - y) \times q$$
where $y$ is the number of clients who will have a yes response at that node. 
%How to estimate the number of "yesses" before do query ??
Since we have not sent a query yet, we can approximate this by one of the following:
\begin{itemize}
    \item Maximum count: $y = |\mathcal{A}|$
    \item Minimum count: 0
    \item Parent count
    \item Cutoff threshold: $y = \lambda \times |\mathcal{A}|$
    \item Randomly select a count between 0 and $|\mathcal{A}|$
\end{itemize}
We note that this may not be the most accurate way to estimate $y$ but at this point we only need an \textit{approximation} to determine how much budget we should use for this query. Later, as shown in next steps we will account for the added noise in our query after the query has been sent.

\Jnote{Changed this to be $\mathcal{V}$ ... should this still be $\lambda$ ?}
Given our estimated count $\hat{c}$, we wish to find the confidence interval for which the true count $c$ is $\leq \mathcal{V}$. We formulate this as:
$$CI = \int_{x=0}^{\mathcal{V}} P[c=x \;\lvert\; \hat{c}]$$
% CI\_high = 1 - CI\_low
which can be solved using a PDF (assuming a continuous distribution) or by the summation of the probabilities at each value of $x$.

Therefore, the final optimization problem we solve for to find $\beta$ is as follows, where $\theta$ is the confidence interval hyperparameter (e.g., 95\%):
$$\min_{\beta} \quad CI \geq \theta$$
$$\min_{\beta} \quad \left(\int_{x=0}^{\mathcal{V}} P[c=x \;\lvert\; \hat{c}] \right) \geq \theta$$
$$\min_{\beta} \quad \left(\int_{x=0}^{\mathcal{V}} P[c=x \;\lvert\; (y \times p + (\mathcal{A} - y) \times q)] \right)  \geq \theta$$
$$\min_{\beta} \quad \left(\int_{x=0}^{\mathcal{V}} P[c=x \;\lvert\; (y \times \frac{e^\beta}{1 + e^\beta} + (\mathcal{A} - y) \times (\frac{1}{1 + e^\beta})))] \right) \geq \theta$$
% $$\min_{\beta} CI\_low \geq \theta \; or \; CI\_high \geq \theta$$

\noindent Essentially, find the minimum budget that allows us to prune or don't prune branch with high confidence ($\theta$).


\textbf{After query sent:} 
After we have sent our query, based on the client response plus its history of responses, and $p$ and $q$ (random response noise parameters), we can calculate the probability that they have a true match to the template. We define the returned client response as $\mathtt{R}$, and the client true response as $\mathtt{T}$. Based on the client response, we wish to calculate either $P(\mathtt{T}=1|\mathtt{R}=1)$ or $P(\mathtt{T}=1|\mathtt{R}=0)$. We formulate these as follows:
\begin{equation}
\begin{split}
&P(\mathtt{T}=1|\mathtt{R}=1)\\
&= \frac{P(\mathtt{R}=1|\mathtt{T}=1)P(\mathtt{T}=1)}{P(\mathtt{R}=1|\mathtt{T}=1)P(\mathtt{T}=1) + P(\mathtt{R}=1|\mathtt{T}=0)P(\mathtt{T}=0)}\\
&= \frac{p\omega \times \omega}{p\omega \times \omega + (1-p)q \times (1-\omega)}
\end{split}
\end{equation}
\begin{equation}
\begin{split}
&P(\mathtt{T}=1|\mathtt{R}=0)\\
&= \frac{P(\mathtt{R}=0|\mathtt{T}=1)P(\mathtt{T}=1)}{P(\mathtt{R}=0|\mathtt{T}=1)P(\mathtt{T}=1) + P(\mathtt{R}=0|\mathtt{T}=0)P(\mathtt{T}=0)}\\
&= \frac{(1-p)q \times \omega}{(1-p)q \times \omega + p(1-\omega) \times (1-\omega)}
\end{split}
\end{equation}
where $\omega$ is the prior probability of a true yes response, which comes from the history of client queries. Explicitly, this is the previously estimated $y$ yes response count from the previous query of this client on that node. If no previous query, assume $\omega = 0.5$ (50\% chance of returning a yes or no). 

Based on this computation we do two things: (1) Compute a confidence interval to determine whether or not we should prune this branch and (2) update the set of active clients at this node.

%This is a personalized analysis - don't need this for holistic computation
\textit{Pruning:} Based on this interval, we determine whether or not to prune.
\Jnote{Remove $\lambda$}
% Valid rule threshold $\mathcal{V}$ vs cutoff/pruning threshold $\lambda$
We have a valid rule threshold $\mathcal{V}$ and our cutoff/pruning threshold $\lambda$. Currently, $\lambda = \mathcal{V}$ but this does not need to be the case, and you could have a more strict or lenient $\lambda$ based on a chosen trade-off between noise addition and pruning accuracy; e.g., can use more noise and be less eager to cutoff or use less noise and be more eager to cutoff. 
% (cutoff more aggressively or use less budget in the query).

Using the list of individual probabilities, we can compute the probability the true count $c_T \leq \lambda$: %a confidence threshold that all of the clients have true matches to the template and 

$$P(c_T \leq \lambda) = \sum_{k=0}^{\lambda \times n} {n \choose k} \times \left( \prod_{i \in n}(1 - pr_i) \right)$$
where $\lambda \times n$ gives the count needed to meet the cutoff threshold, and $pr_i$ is the individual probability of a true match for client $i$.
Then we prune the branch if: 
$$P(c_T \leq \lambda) \geq \theta$$
i.e., prune if we have high confidence that the true count is $\leq$ the cutoff threshold $\lambda$.
% \Jnote{Does this make sense ...?}
% \Jnote{Does it make sense to aggregate our \textit{individual} computed probabilities or should this be done as a whole for the distribution (e.g., using the responses we get back and p and q holistically) and then do the individual computations only for determining the active clients ... ?}

%ACTIVE CLIENTS
\textit{Active Clients:}
We remove the client from the set of active clients if its probability of a true match is below $1-\theta$, the confidence/error hyperparameter (e.g., 95\%). %the cutoff threshold $\lambda$.
From there, the client is removed from the active client list if $\mathtt{R}=1$ and $P(\mathtt{T}=1|\mathtt{R}=1) < (1-\theta)$ or $\mathtt{R}=0$ and $P(\mathtt{T}=1|\mathtt{R}=0) < (1-\theta)$.



% % Various notes about pruning steps
% Can adjust the cutoff and the noise
% For given beta and V, ensure that likelihood cutting off when true value actually less than lambda is 5\%

% % Can use more noise and be less eager to cutoff or use less noise and be more eager to cutoff (cutoff more aggressively or use less budget in the query)
% Pruning: Based on sent query, responses and noise we used, determine whether we should actually cutoff this branch or not:
% Compute likelihood that true count is actually less than lambda --> if this so with 95\% confidence then cut off, if not, don't cut off
% Compute this based on \# A, noise added (p and q) and responses we got ...

% Cutoff if 95\% of the true clients below threshold

% Given query and distribution of responses on that query, what is prob cutoff incorrectly? If cutoff exactly at lambda

% Problem solving: if true value V, what cutoff needed to make <5\% error that we cutoff according to V (e.g., what do we set lambda to?) Then, if get to chosen lambda cut off or not

% How willing are we to miss a valid rule?
% How far above or below lambda does our count need to be before we get below the 5\% threshold? (how much noise can we handle?)

% If count at lambda with nonzero noise, have probability 1/2 we cutoff, this assuming <= lambda cutoff
% Most sensitive case is 1 above cutoff or 1 below

% If true value 0 want to maximize cutoff, if true value above then want to minimize cutoff prob

% Based on all of this and tolerance for failures (error prob) compute whether to cutoff or not
% -- either can get confidence threshold based on query and noise and V; if 95\% confident that true value actually < lamdba then cutoff, else don't (even if noisy count < lambda) OR
% -- compute what lambda we actually need (e.g. could be larger than V) to ensure that we cutoff with 95\% confidence --> then if our resp count is < lambda cutoff, else don't


% \textbf{Active Clients.} 
% After we have sent a query: update the set of active clients based on their responses.
% One of the biggest updates in the private model is how to determine when clients are still active or not, since clients do not always respond truthfully anymore. At each query of a rule structure, we query the set of active clients, and then for each client, based on the response the client returns plus its history of responses, we calculate the probability that they have a true match, $y_{true}$ to the template. We remove the client from the set of active clients if its probability of a true match is below the cutoff threshold $\lambda$. We define the returned client response as $\mathtt{R}$, and the client true response as $\mathtt{T}$. Based on the client response, we wish to calculate either $P(\mathtt{T}=1|\mathtt{R}=1)$ or $P(\mathtt{T}=1|\mathtt{R}=0)$. We can formulate these as follows, based on the randomized response protocol~\cite{wang2017locally}:
% \begin{equation}
% \begin{split}
% &P(\mathtt{T}=1|\mathtt{R}=1)\\
% &= \frac{P(\mathtt{R}=1|\mathtt{T}=1)P(\mathtt{T}=1)}{P(\mathtt{R}=1|\mathtt{T}=1)P(\mathtt{T}=1) + P(\mathtt{R}=1|\mathtt{T}=0)P(\mathtt{T}=0)}\\
% &= \frac{p\theta \times \theta}{p\theta \times \theta + (1-p)q \times (1-\theta)}
% \end{split}
% \end{equation}
% \begin{equation}
% \begin{split}
% &P(\mathtt{T}=1|\mathtt{R}=0)\\
% &= \frac{P(\mathtt{R}=0|\mathtt{T}=1)P(\mathtt{T}=1)}{P(\mathtt{R}=0|\mathtt{T}=1)P(\mathtt{T}=1) + P(\mathtt{R}=0|\mathtt{T}=0)P(\mathtt{T}=0)}\\
% &= \frac{(1-p)q \times \theta}{(1-p)q \times \theta + p(1-\theta) \times (1-\theta)}
% \end{split}
% \end{equation}
% where $\theta$ is the prior probability of a true yes response, which comes from the history of client queries. Explicitly, this is the previously estimated $\mathcal{Y}$ yes response count from the previous query of this client on that node. If no previous query, assume $\theta = 0.5$ (50\% chance of returning a yes or no). From there, the client is removed from the active client list if $\mathtt{R}=1$ and $P(\mathtt{T}=1|\mathtt{R}=1) \le \lambda$ or $\mathtt{R}=0$ and $P(\mathtt{T}=1|\mathtt{R}=0) \le \lambda$.



%%%% V6 leftovers

\textbf{Baseline.} In the baseline method, use a uniform budget for every query by dividing the total privacy budget by the number of user specified queries: $\beta = \epsilon/Q$, where $Q$ is the total number of queries.

A user $i$ outputs a response $r_i$, which is equal to the true value or heads with value $p$ and a random value or tails with probability q (uniformly at random): 
$$p = \frac{e^\beta}{1 + e^\beta}, \quad q = 1-p = \frac{1}{1 + e^\beta}$$ 


% V6
%%%%%%%%%%%%%% ADAPTIVE PROTOCOL OVERVIEW %%%%%%%%%%%%%%
\begin{algorithm}
\caption{Adaptive Budget Protocol}
\label{alg-adptv}
\SetAlgoLined
\DontPrintSemicolon
\SetNoFillComment
\SetKwProg{Fn}{Function}{:}{end}
\SetKwFunction{pruneTree}{PruneTree}
% \Fn{\pruneTree{template tree $T$, cutoff threshold $\lambda$}}
{
    Before query: $\beta \leftarrow$ FindBudget($\mathcal{V}, n$) \;
    Send query: $y \leftarrow$ Query($\beta$, n) \;
    Correct query count: $c = (y - nq) / (p-q)$ \;
    After query: PruneTree($\hat{c}, n, \beta$) \;
    UpdateActiveClients(y_c, $\beta$) \;
}
\end{algorithm}
% Before Query: Estimate budget per query. Beta
% After Query: Based on randomized response parameters and responses …
%   Determine whether or not to prune this branch
%   Update active clients

\newpage 
\textbf{Before query: Determine Ploss budget for this query, $\beta$}
% \textbf{Before query sent: estimate budget $\beta$ to use}
% Before we send our next query: find the optimal budget per query $\beta$ that allows us to prune branches with high confidence.
Given the set of clients $n$, the true count $c$, and the valid rule threshold $\mathcal{V}$, 
we can get an estimate count of yes responses $\hat{c}$ based on a selected $\beta$:
% $$\hat{c} = y \times p + (n - y) \times q$$
$$\hat{c} = y \times \frac{e^\beta}{1 + e^\beta} + (n - y) \times \frac{1}{1 + e^\beta}$$
where $y$ is the number of clients who will have a yes response at that node. We don't know $y$ yet since we have not sent a query yet (don't have the user responses.)

% Therefore, we wish to estimate: assuming our true count is the worst case where $c = \mathcal{V}$, where we right at boundary but should not prune, as close as possible to prune boundary without pruning, what is the probability we cutoff? 
We assume our true count $c$ is the worst case, where $c = \mathcal{V}$, at the boundary of our pruning threshold. We wish to find the smallest budget that allows us to prune 
% or don't prune branch 
with high confidence ($\theta$):
\begin{align*}
\min_{\beta} \quad & P(\hat{c} < \mathcal{V} | c, n) \geq \theta \\
\min_{\beta} \quad & \left(\int_{y=0}^{n} P(\hat{c} < \mathcal{V} | c, n) \right) \geq \theta \\
\min_{\beta} \quad & \left(\int_{y=0}^{n} P((y \times \frac{e^\beta}{1 + e^\beta} + (n - y) \times \frac{1}{1 + e^\beta}) < \mathcal{V} | c, n) \right) \geq \theta \\
\min_{\beta} \quad & \left(\int_{y=0}^{n} PDF(y, c, \sigma_c) \right) \geq \theta
\end{align*}



\Jnote{Should we integrate through all possible values of y, so from 0 to n? Or just 0 to $\mathcal{V}$ is okay?}

\Jnote{Does it make sense to have this be a theorem? Definition...?}
% Given our estimated count $\hat{c}$, we wish to find the confidence interval for which the true count $c$ is $\leq \mathcal{V}$. We formulate this as:
% $$CI = \int_{y=0}^{\mathcal{V}} P[\hat{c}=y \;\lvert\; c]$$
% % CI\_high = 1 - CI\_low
% which can be solved using a PDF (assuming a continuous distribution) or by the summation of the probabilities at each value of $x$.

% Therefore, the final optimization problem we solve for to find $\beta$ is as follows, where $\theta$ is the confidence interval hyperparameter (e.g., 95\%):
% $$\min_{\beta} \quad CI \geq \theta$$
% $$\min_{\beta} \quad \left(\int_{x=0}^{\mathcal{V}} P[c=x \;\lvert\; \hat{c}] \right) \geq \theta$$
% $$\min_{\beta} \quad \left(\int_{x=0}^{\mathcal{V}} P[c=x \;\lvert\; (y \times p + (\mathcal{A} - y) \times q)] \right)  \geq \theta$$
% $$\min_{\beta} \quad \left(\int_{x=0}^{\mathcal{V}} P[c=x \;\lvert\; (y \times \frac{e^\beta}{1 + e^\beta} + (\mathcal{A} - y) \times (\frac{1}{1 + e^\beta})))] \right) \geq \theta$$
% % $$\min_{\beta} CI\_low \geq \theta \; or \; CI\_high \geq \theta$$

\noindent \textbf{Send Query:} Using budget $\beta$, get a count of how many clients have a rule match
\newline

\noindent \textbf{After Query Sent:}
\begin{definition}[Pruning]
After the query sent, given the estimated count $\hat{c}$, $n$ and $\beta$, prune this branch if there is high confidence ($\theta$) that the true count $c$ is less than the valid rule threshold $\mathcal{V}$:
$$P(c < \mathcal{V} | \hat{c}, \beta, n) \geq \theta$$
\end{definition}

\Jnote{Based on the responses I get, $y$, I \textit{correct} this count based on what I know about the protocol and the noise added to get an "Unbiased estimate" of the true count. Is this sufficient for this probability?? Or do I need to compute a separate probability measure based on the noise etc ...?}


% \Jnote{This formulation needs to now be simplified just assuming a centralized Gaussian distribution - just compute noise impact from basic randomized response protocol, should be in basic lit to reference and can do this with basic PDF ..}
% % OLD formulation
% Using the list of individual probabilities, we can compute the probability the true count $c_T \leq \lambda$: %a confidence threshold that all of the clients have true matches to the template and 

% $$P(c_T \leq \lambda) = \sum_{k=0}^{\lambda \times n} {n \choose k} \times \left( \prod_{i \in n}(1 - pr_i) \right)$$
% where $\lambda \times n$ gives the count needed to meet the cutoff threshold, and $pr_i$ is the individual probability of a true match for client $i$.
% Then we prune the branch if: 
% $$P(c_T \leq \lambda) \geq \theta$$
% i.e., prune if we have high confidence that the true count is $\leq$ the cutoff threshold $\lambda$.
% % \Jnote{Does this make sense ...?}
% % \Jnote{Does it make sense to aggregate our \textit{individual} computed probabilities or should this be done as a whole for the distribution (e.g., using the responses we get back and p and q holistically) and then do the individual computations only for determining the active clients ... ?}




\textbf{Active Clients}
After we have sent our query, based on the client response plus its history of responses, and $p$ and $q$ (random response noise parameters), we can calculate the probability that they have a true match to the template. We define the returned client response as $\mathtt{R}$, and the client true response as $\mathtt{T}$. Based on the client response, we wish to calculate either $P(\mathtt{T}=1|\mathtt{R}=1)$ or $P(\mathtt{T}=1|\mathtt{R}=0)$. We formulate these as follows:
\begin{equation}
\begin{split}
&P(\mathtt{T}=1|\mathtt{R}=1)\\
&= \frac{P(\mathtt{R}=1|\mathtt{T}=1)P(\mathtt{T}=1)}{P(\mathtt{R}=1|\mathtt{T}=1)P(\mathtt{T}=1) + P(\mathtt{R}=1|\mathtt{T}=0)P(\mathtt{T}=0)}\\
&= \frac{p\omega \times \omega}{p\omega \times \omega + (1-p)q \times (1-\omega)}
\end{split}
\end{equation}
\begin{equation}
\begin{split}
&P(\mathtt{T}=1|\mathtt{R}=0)\\
&= \frac{P(\mathtt{R}=0|\mathtt{T}=1)P(\mathtt{T}=1)}{P(\mathtt{R}=0|\mathtt{T}=1)P(\mathtt{T}=1) + P(\mathtt{R}=0|\mathtt{T}=0)P(\mathtt{T}=0)}\\
&= \frac{(1-p)q \times \omega}{(1-p)q \times \omega + p(1-\omega) \times (1-\omega)}
\end{split}
\end{equation}
where $\omega$ is the prior probability of a true yes response, which comes from the history of client queries. Explicitly, this is the previously estimated $y$ yes response count from the previous query of this client on that node. If no previous query, assume $\omega = 0.5$ (50\% chance of returning a yes or no). 

We remove the client from the set of active clients if its probability of a true match is below $1-\theta$, the confidence/error hyperparameter (e.g., 95\%). %the cutoff threshold $\lambda$.
From there, the client is removed from the active client list if $\mathtt{R}=1$ and $P(\mathtt{T}=1|\mathtt{R}=1) < (1-\theta)$ or $\mathtt{R}=0$ and $P(\mathtt{T}=1|\mathtt{R}=0) < (1-\theta)$.



% Notes about analysis --> will need to analyze worse case for branch searching ...
Analysis of worst case --> V patients have the rule with no other branches 
Could be something to analyze

In the worst case have some prob of getting rule but the error hyperparam can be different 
Deepest rules with most operators

What rules are not learned and why ...? --> what i



FindCutoffThresh($\beta, \mathcal{V}, n, \hat{c}$):
The true count can be calculated as:
$$c = \frac{\hat{c} - nq}{p-q}$$
$$\sigma_c = \frac{nq(1-q)}{(p-q)^2}$$
Since $c$ is the sum of many independent random responses, its distribution is very close to a normal distribution~\cite{wang2017locally}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% V6

We define the true (unknown) count as $c$ and the estimated count as $\hat{c}$. 
Important assumptions: since our responses are the sum of many independent random responses, its distribution is very close to a normal distribution~\cite{wang2017locally}. Moreover, we know that $E[\hat{c}] = c$. We are also always assuming the worst case where the true count $c = \mathcal{V}$ for all calculations.


% \textbf{Baseline.} In the baseline method, use a uniform budget for every query by dividing the total privacy budget by the number of user specified queries: $\beta = \epsilon/Q$, where $Q$ is the total number of queries.

% A user $i$ outputs a response $r_i$, which is equal to the true value or heads with value $p$ and a random value or tails with probability q (uniformly at random): 
% $$p = \frac{e^\beta}{1 + e^\beta}, \quad q = 1-p = \frac{1}{1 + e^\beta}$$ 


% V6
%%%%%%%%%%%%%% Rule Discovery Protocol %%%%%%%%%%%%%% 
\begin{algorithm}
\caption{Rule Discovery Protocol}
\SetAlgoLined
\DontPrintSemicolon
\SetNoFillComment
% \SetKwInput{KwInput}{Input} 
% \SetKwInput{KwOutput}{Output}
\SetKwProg{Fn}{Function}{:}{end}
\SetKwProg{SubFn}{Sub-Function}{:}{end}
% Set Function Names
\SetKwFunction{FMain}{RunProtocol}
\SetKwFunction{selection}{Selection}
\SetKwFunction{expansion}{Expansion}
\SetKwFunction{getQuery}{GetQuery}
\SetKwFunction{backprop}{Backpropagation}
\SetKwFunction{pruneTree}{PruneTree}
\SetKwFunction{selectchildnode}{selectChildnode}
\SetKwFunction{adptvProt}{Adaptive Budget Protocol}
\SetKwFunction{findCutoff}{Prune\_Branch}
\SetKwFunction{CDF}{CDF}
\SetKwFunction{findBeta}{FindBeta}
\SetKwFunction{errorProb}{Compute\_Error\_Prob}
\SetKwFunction{query}{SendQuery}
\label{alg-protocol-overview}
\Fn{\FMain{template tree $T$, valid rule threshold $\mathcal{V}$, number of clients $n$, error threshold $\theta$}}{
    $b \longleftarrow$ $T.root$\; %was currentnode
    \Repeat{budget used or tree completely explored}{ %was while
        $b_{selected}$ $\longleftarrow$ \selection{b}\;
        $b_{expanded}$ $\longleftarrow$ \expansion{$b_{selected}$}\;
        \eIf{$b_{expanded}$ $\neq$ None}{
            $b$ $\longleftarrow$ $b_{expanded}$
        }
        {
            $b$ $\longleftarrow$ $b_{selected}$
        }
        
        $\beta \leftarrow$ \findBeta{$\mathcal{V}, n, \theta$} \tcp{Get budget per query}
        %make these ones implicit, don't mention here
        $p \longleftarrow \frac{e^\beta}{1 + e^\beta}$ \tcp{Prob respond truthfully, from rand resp protocol}
        $q \longleftarrow 1-p = \frac{1}{1 + e^\beta}$ \tcp{Prob respond randomly, from rand resp  protocol}
        
        \For{$cl$ in $n$ clients}{ \tcp{Query all the clients}
            $y$ +=  $cl$.\query{$b, \beta$}\;
        }
        $\hat{c} \longleftarrow \frac{y - nq}{p-q}$ \tcp{Compute the unbiased estimate of the count }
        $\sigma_c \longleftarrow \frac{nq(1-q)}{(p-q)^2}$ \tcp{Compute std dev of $c$}

        Find $\lambda$ s.t. $P(\hat{c} < \mathcal{V} + \lambda \;\lvert\; c = \mathcal{V}) > \theta$ \;
        \tcc{Compute this probability using \CDF{$\mathcal{V} + \lambda - \hat{c}, c, \sigma_c$}}
        \If{$\hat{c} < \mathcal{V} + \lambda$}{\pruneTree($b$, $T$)}
        \backprop{$b$, $\hat{c}$}\;
        % \pruneTree{$T$, $\lambda$} 
    }
    $R_S \longleftarrow$ $T$.generateRuleset()\;
    \Return population ruleset $R_S$\;
}
\end{algorithm}

\newpage
Find $\beta$: The point of this equation is to find the optimal budget per query $\beta$ that allows us to prune branches with high confidence:
\begin{align}
    &p \longleftarrow \frac{e^\beta}{1 + e^\beta} \\
    &q \longleftarrow 1-p = \frac{1}{1 + e^\beta} \\
    &\hat{c} = y \times p + (n - y) \times q \\
    &\min_{\beta} \left( \int_{y=0}^{n} (P(\hat{c} < \mathcal{V} \;\lvert\; c = \mathcal{V}) ) \right) \geq \theta 
    % Compute this probability using \CDF{$\mathcal{V} - \hat{c}, c, \sigma_c$}
    % Computed CDF($x \;\lvert\; \mu, \sigma$)
\end{align}



% \begin{algorithm}
% \caption{Find Beta}
% \label{alg-find-beta}
% \SetAlgoLined
% \DontPrintSemicolon
% \SetNoFillComment
% \SetKwProg{Fn}{Function}{:}{end}
% \Fn{\findBeta{valid rule threshold $\mathcal{V}$, number of clients $n$, error threshold $\theta$}}{
%     $$\min_{\beta} \left( \int_{y=0}^{n} (\text{\errorProb{$\beta, \mathcal{V}, n, y$}} ) \right) \geq \theta$$ 
%     \Return $\beta$
% }
% \Fn{\errorProb{budget $\beta$, valid rule threshold $\mathcal{V}$, number of clients $n$, number of yes responses $y$}}{
%     $p \longleftarrow \frac{e^\beta}{1 + e^\beta}$ \tcp{Prob respond truthfully, from rand resp protocol}
%     $q \longleftarrow 1-p = \frac{1}{1 + e^\beta}$ \tcp{Prob respond randomly, from rand resp protocol}
%     $\hat{c} = y \times p + (n - y) \times q$ \tcp{Compute estimated count}
%     $\sigma_c \longleftarrow \frac{nq(1-q)}{(p-q)^2}$ \tcp{Compute std dev of $c$}
%     \Return $P(\hat{c} < \mathcal{V} \;\lvert\; c = \mathcal{V})$ \tcp{Compute this probability using \CDF{$\mathcal{V} - \hat{c}, c, \sigma_c$}}
% }
% \end{algorithm}


% \begin{algorithm}
% \caption{Adaptive Pruning}
% \label{alg-pruning}
% \SetAlgoLined
% \DontPrintSemicolon
% \SetNoFillComment
% \SetKwProg{Fn}{Function}{:}{end}
% \Fn{\findCutoff{budget $\beta$, valid rule threshold $\mathcal{V}$, number of clients $n$, number of yes responses $y$, error threshold $\theta$}}{
%     % Given $\hat{c} < \mathcal{V}$, should we cut off or not? Find the threshold needed to ensure we cut off with 95\% confidence \;
%     % Find a cutoff threshold such that the probability of cutting off incorrectly (when the true count is <= V) is less than $\theta$? \;
%     $p \longleftarrow \frac{e^\beta}{1 + e^\beta}$ \tcp{Prob respond truthfully, from rand resp protocol}
%     $q \longleftarrow 1-p = \frac{1}{1 + e^\beta}$ \tcp{Prob respond randomly, from rand resp  protocol}
%     $\hat{c} \longleftarrow \frac{y - nq}{p-q}$ \tcp{Compute the unbiased estimate of the count }
%     $\sigma_c \longleftarrow \frac{nq(1-q)}{(p-q)^2}$ \tcp{Compute std dev of $c$}
%     % $z = \frac{\mathcal{V} - c}{\sigma_c}$ \;
%     % $P(\hat{c} < \mathcal{V} \;\lvert\; c = \mathcal{V})$ \tcp{Use the probability density function (PDF) to find this probability since we know $E[\hat{c}] = c$ and $\sigma_c$}
%     Find $\lambda$ s.t. $P(\hat{c} < \mathcal{V} + \lambda \;\lvert\; c = \mathcal{V}) > \theta$ \;
%     \tcc{Compute this probability using \CDF{$\mathcal{V} + \lambda - \hat{c}, c, \sigma_c$}}
%     \uIf{$\hat{c} < \mathcal{V} + \lambda$}{Prune branch}
%     \Else{Don't Prune}
%     % \Return $\mathcal{V} + ?$ \tcp{Return threshold needed to prune, and if should prune or not} 
% }
% \Fn{\CDF{value $x$, mean distribution centered at $\mu$, standard deviation distribution centered at $\sigma$}}{
%     \Return Computed CDF($x \;\lvert\; \mu, \sigma$)
% }
% \end{algorithm}









% \textbf{Active Clients}
% After we have sent our query, based on the client response plus its history of responses, and $p$ and $q$ (random response noise parameters), we can calculate the probability that they have a true match to the template. We define the returned client response as $\mathtt{R}$, and the client true response as $\mathtt{T}$. Based on the client response, we wish to calculate either $P(\mathtt{T}=1|\mathtt{R}=1)$ or $P(\mathtt{T}=1|\mathtt{R}=0)$. We formulate these as follows:
% \begin{equation}
% \begin{split}
% &P(\mathtt{T}=1|\mathtt{R}=1)\\
% &= \frac{P(\mathtt{R}=1|\mathtt{T}=1)P(\mathtt{T}=1)}{P(\mathtt{R}=1|\mathtt{T}=1)P(\mathtt{T}=1) + P(\mathtt{R}=1|\mathtt{T}=0)P(\mathtt{T}=0)}\\
% &= \frac{p\omega \times \omega}{p\omega \times \omega + (1-p)q \times (1-\omega)}
% \end{split}
% \end{equation}
% \begin{equation}
% \begin{split}
% &P(\mathtt{T}=1|\mathtt{R}=0)\\
% &= \frac{P(\mathtt{R}=0|\mathtt{T}=1)P(\mathtt{T}=1)}{P(\mathtt{R}=0|\mathtt{T}=1)P(\mathtt{T}=1) + P(\mathtt{R}=0|\mathtt{T}=0)P(\mathtt{T}=0)}\\
% &= \frac{(1-p)q \times \omega}{(1-p)q \times \omega + p(1-\omega) \times (1-\omega)}
% \end{split}
% \end{equation}
% where $\omega$ is the prior probability of a true yes response, which comes from the history of client queries. Explicitly, this is the previously estimated $y$ yes response count from the previous query of this client on that node. If no previous query, assume $\omega = 0.5$ (50\% chance of returning a yes or no). 

% We remove the client from the set of active clients if its probability of a true match is below $1-\theta$, the confidence/error hyperparameter (e.g., 95\%). %the cutoff threshold $\lambda$.
% From there, the client is removed from the active client list if $\mathtt{R}=1$ and $P(\mathtt{T}=1|\mathtt{R}=1) < (1-\theta)$ or $\mathtt{R}=0$ and $P(\mathtt{T}=1|\mathtt{R}=0) < (1-\theta)$.


